Beyond Natural Language: LLMs Leveraging Alternative Formats for Enhanced Reasoning and Communication

Natural language (NL) has long been the predominant format for human cognition and communication, and by extension, has been similarly pivotal in the development and application of Large Language Models (LLMs). Yet, besides NL, LLMs have seen various non-NL formats during pre-training, such as code and logical expression. NL's status as the optimal format for LLMs, particularly in single-LLM reasoning and multi-agent communication, has not been thoroughly examined. In this work, we challenge the default use of NL by exploring the utility of non-NL formats in these contexts. We show that allowing LLMs to autonomously select the most suitable format before reasoning or communicating leads to a 3.3 to 5.7\% improvement in reasoning efficiency for different LLMs, and up to a 72.7\% reduction in token usage in multi-agent communication, all while maintaining communicative effectiveness. Our comprehensive analysis further reveals that LLMs can devise a format from limited task instructions and that the devised format is effectively transferable across different LLMs. Intriguingly, the structured communication format decided by LLMs exhibits notable parallels with established agent communication languages, suggesting a natural evolution towards efficient, structured communication in agent communication. Our code is released at \url{https://github.com/thunlp/AutoForm}.

==> sections/analysis.tex <==
\section{Analysis}
\label{sec:analysis}

Following the presentation of our experimental results, we would like to delve deeper into understanding the implications and nuances of our findings. The experimental results in the last section have clearly demonstrated that allowing LLMs to autonomously decide on the thought or communication format results in enhanced reasoning and more efficient communication. To further elucidate these outcomes, we engage in a comprehensive analysis addressing several pivotal research questions (RQ). These questions aim to unravel the intricacies of format selection by LLMs and its impact on task performance across different scenarios:
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/medium.pdf}
    \vspace{-0.8em}
    \caption{Format distribution chosen by Gemini Pro (a), GPT-3.5 (b) and GPT-4 (c), and the overall format distribution across tasks from both models (d).}
    \label{fig:media-dist}
    % \vspace{-1em}
\end{figure*}
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=1em]
    \item \textbf{RQ1}: What formats are chosen in single-LLM reasoning?~(\cref{sec:analysis-chosen-media})
    \item \textbf{RQ2}: Can LLMs devise a general format for a task based on some task inputs?~(\cref{sec:analysis-medium-generalization})
    \item \textbf{RQ3}: Is the decided format transferable between different LLMs?~(\cref{sec:analysis-transferability})
    \item \textbf{RQ4}: What are the features of the formats used in multi-agent communication? ~(\cref{sec:analysis-comm-features})
    \item \textbf{RQ5}: Does the autonomously determined multi-agent communication format align with conventional agent communication languages such as KQML~\citep{DBLP:conf/cikm/FininFMM94}?~(\cref{sec:analysis-comm-acl})
\end{itemize}

\input{tables/seprated-automed}
\subsection{RQ1: Formats Chosen in Single-LLM Reasoning}
\label{sec:analysis-chosen-media}
In addressing RQ1, we investigate the formats selected from LLMs when tasked with reasoning. This analysis is pivotal in understanding how LLMs, when granted the autonomy to choose, navigate away from the default NL format to potentially more efficient alternatives.

% To conduct this investigation, we randomly sample 50 examples from each dataset and examine the reasoning traces generated using AutoMed, as reported in~\cref{tab:multi-exp-results}. The distribution of the chosen mediums by different LLMs across various datasets is illustrated in the pie chart in~\cref{fig:???}. Our findings reveal a rich variety of media preferences among LLMs. While a significant number of instances continue to utilize NL, owing to its inherent flexibility and expressiveness, we observed a marked preference for structured formats such as markdown tables, lists, and logical operators. This trend is particularly pronounced in tasks requiring logical reasoning, where these formats provide a clearer and more succinct representation of information.

We analyze a randomly sampled set of 50 examples from each dataset, investigate the reasoning traces produced with AutoForm, and manually count the number of appeared formats. \cref{fig:media-dist}(a-c) display the distribution of formats chosen by Gemini Pro, GPT-3.5 and GPT-4, and \cref{fig:media-dist}(d) displays their combined preferences across various tasks. The data indicates a notable diversity in format selection by LLMs. A shift towards structured formats, such as lists, logical expressions, and markdown tables is observed. These formats are particularly favored in tasks that demand logical reasoning, offering clearer and more concise data representation, as illustrated in~\cref{fig:media-dist}(d).


\subsection{RQ2: Generalization of Format Selection Based on Task Inputs}
\label{sec:analysis-medium-generalization}
% In the experiments we have done so far, the LLMs decide the medium implicitly for each given instruction, as elaborated in~\cref{sec:method-medium-choosing}. Intuitively, a task often has a medium that is generally appropriate to the task. Instead of implicitly letting the LLMs decide the medium, we make AutoMed a two-step approach: 1) task the LLM with identifying the most efficient medium given the problem(s); 2) use the medium to solve the problem. We term this approach \textbf{two-step AutoMed}. Using this method, we can try to answer RQ3, exploring the possibility of deciding on a general medium for a specific task.

An examination of~\cref{fig:media-dist}(d) reveals a discernible variation in the LLMs' format preferences across different tasks. This variation aligns with the expectation that the optimal format would naturally differ between tasks, each with its unique requirements. In addressing RQ2, we probe whether LLMs are capable of identifying a general format suitable for a given task based on a subset of inputs, and then consistently applying this format for problem-solving. In AutoForm, as delineated in~\cref{sec:method-medium-choosing}, LLMs typically select a format \textit{implicitly} for each instruction on a case-by-case basis. Nonetheless, it stands to reason that certain tasks may be inherently conducive to a specific format. To investigate this hypothesis, we introduce the \textbf{two-step AutoForm}. This approach tasks an LLM with first determining the most efficient format and subsequently utilizing that format in the CoT problem-solving stage. That is, we turn the implicit format decision into an explicit step, which mathematically follows~\cref{eq:cot-formula} instead of merging the two steps.



The two-step AutoForm experiments with two distinct settings: 1) \textit{Instance-Based}, where the LLM selects a format for each instruction, and 2) \textit{Task-Based}, where the LLM deduces a general format for the entire task by analyzing 5 inputs from the task. Note that, unlike few-shot prompting, the Task-Based setting does not provide answers within the inputs, and these inputs are only utilized during the format decision step. 

The results are detailed in \cref{tab:two-step-automed}. The Task-Based setting demonstrates that both GPT-3.5 and Gemini Pro can effectively generalize a thought format from a limited set of inputs within a task, and often outperforming the Instance-Based setting. In contrast, GPT-4 shows similar performance levels in both Task-Based and Instance-Based settings, suggesting that its advanced capabilities may afford it greater flexibility in format usage. These findings indicate that LLMs, particularly less sophisticated ones like GPT-3.5, may benefit from exposure to multiple inputs from a task to better generalize an effective thought format. This ability of LLMs to generalize the format for a task makes the AutoForm approach more practical since the format can be identified only once for a specific task.


% We employed two-step AutoMed under two distinct settings: \textit{Instance-Based}, where the LLM selects a medium for each instruction individually, and \textit{Task-Based}, where the LLM determines a general medium for the task after analyzing five examples. Note that the difference between Task-Based setting and few-shot prompting is that Task-Based setting does not include the answer, and the examples are only visible at the medium decision step. The results are presented in the upper two groups of~\cref{tab:two-step-automed}. For GPT-3.5, the medium determined in Task-Based setting brings even better performance to the model, while for GPT-4, the performance of Instance-Based and Task-Based settings are comparable. The results indicate that given several instances from a task, LLMs can generalize a medium across a task. This finding makes AutoMed more practical, as the medium can be generated once and for all for a specific task, greatly saving the token usage.
% In this subsection, we explore the potential of LLMs to generalize a medium for a task based on a set of examples, addressing RQ3. We introduce a novel method, termed "Two-Stage Media Adaptation (TSMA)", to investigate whether the medium selection by LLMs is instance-specific or can be generalized across a task. This method is divided into two stages: the first involves determining the medium, and the second applies this medium to solve the problem.

\begin{figure*}[t]
    \vspace{1mm}
    \centering
    \includegraphics[width=0.9\textwidth]{figs/case.pdf}
    \vspace{-0.8em}
    \caption{Multi-agent communication examples. The top panel illustrates a traditional natural language conversation, and the bottom panel shows a conversation using AutoForm. Necessary information related to the question is marked in \colorbox{mygreen}{green}, redundant information is marked in \colorbox{myred}{red}, and speech-act-related phrases are marked in \colorbox{myyellow}{orange}.}
    \label{fig:case}
    % \vspace{-1.3em}
\end{figure*}
\subsection{RQ3: Transferability of Format Across Different LLMs}
\label{sec:analysis-transferability}

% \subsection{Separated AutoMed}
% \label{sec:analysis-separated-automed}

% \paragraph{Extra Experiments}
% To evaluate whether LLM can independently determine an optimal medium for problem-solving, we have revised our methodology into a two-stage process. In the initial stage, the LLM is tasked exclusively with identifying the most efficient medium. We adopted two settings: current and multiple. In the former setting, the LLM is presented with the same task description as that used in the subsequent stage for medium selection. Conversely, in the latter scenario, we randomly selects five entries from the dataset. These entries serve as the basis for generating a medium recommendation. Subsequently, in the second stage, the LLM employs the selected medium format to solve the problem at hand.

This subsection delves into RQ3, the transferability of the format across LLMs. The concept of format transferability is crucial in understanding the universality of formats decisions made by LLMs and their applicability across various models. Instead of using the same model for format selection and problem-solving (homogeneous setting) as we have done in~\cref{sec:analysis-medium-generalization}, we explore the heterogeneous setting of the two-step AutoForm, where different models are employed for the two steps.

% To examine whether different versions of LLMs can enhance their performance by leveraging the medium selection made by another model, we utilize distinct LLMs for each stage: one for selecting the optimal medium and another for executing problem-solving tasks. We experimented with two configurations: employing GPT-4 for medium selection in multiple setting followed by GPT-3.5 for problem resolution, and vice versa. 

% \paragraph{Results}

The results are presented in the last group of~\cref{tab:two-step-automed}. Generally, the format is transferable, but may lead to slightly inferior performances compared to the homogeneous setting. For example, transferring the format decided by GPT-4 to GPT-3.5 or Gemini Pro leads to a decrease compared to the homogeneous setting for the two LLMs in most of the tasks except for Coin Flip. On the other hand, when transferring the format decided by GPT-3.5 to GPT-4, the results are generally comparable to the homogeneous setting for GPT-4. For information essentiality, the format selected by GPT-3.5 is generally less efficient, leading to incomplete problem-solving processes. We give examples in \cref{tab:appendix-info-essen-sep-model-examples-3.5-4,tab:appendix-info-essen-sep-model-examples-4-task-based,tab:appendix-info-essen-sep-model-examples-4-3.5}. For other tasks, the format generated by GPT-3.5 proves adequate and is easily interpreted by GPT-4, resulting in similar performances to the homogeneous setting for GPT-4.


% When utilizing the same LLM for both medium selection and problem-solving, our observations indicated a notable performance enhancement with GPT-3.5. Specifically, when selecting a medium based on multiple entries, GPT-3.5 demonstrated an improved ability to identify a more generalized and cohesive medium suitable for diverse problem-solving scenarios. However, it's noteworthy that GPT-3.5 tended to generate distinct media for each entry during the initial stage of mathematical reasoning tasks. In contrast, when GPT-4 was employed for Separated AutoMed, the performance in both single and multiple entry settings was found to be comparable. Interestingly, the mediums chosen by GPT-4 in both scenarios exhibited similar characteristics, being both generic and unified.

% The scenario involving distinct LLMs for medium selection and problem-solving yielded different outcomes. Utilizing GPT-4 for medium selection and GPT-3.5 for problem-solving, we observed a decrease in performance across most tasks, except for simpler symbolic reasoning tasks. In these tasks, GPT-3.5 could effectively interpret and utilize the medium chosen by GPT-4. However, for more complex tasks, GPT-3.5 struggled to appropriately apply the selected medium. Conversely, when GPT-3.5 was responsible for medium selection and GPT-4 for problem-solving, the results were mixed. For information essentiality tasks, the medium selected by GPT-3.5 was generally less efficient and comprehensive compared to GPT-4's selections. Consequently, problem-solving was sometimes incomplete, and the medium chosen by GPT-3.5 was occasionally disregarded. For other task types, the medium selected by GPT-3.5 proved adequate and was easily interpreted by GPT-4, resulting in similar performance levels to those when GPT-4 selected the medium itself.

\subsection{RQ4: Features of Communication Format}
\label{sec:analysis-comm-features}
In addressing RQ4, this subsection investigates the characteristics of the formats used by language agents in multi-agent communication scenarios. Our goal is to identify key attributes contributing to efficient communication by examining the formats used during their interactions.

We analyze 50 random interaction logs for each dataset and present some cases in~\cref{fig:case} and~\cref{sec:appendix-examples}. Despite some retained characteristics of NL, the communication formats decided via AutoForm display distinct features:

\textbf{Clarity and Structure.}
An important feature of the selected formats is an emphasis on clarity. LLMs consistently favor formats facilitating unambiguous and straightforward communication, which is vital in our multi-agent scenarios. In these scenarios, agents possess divergent knowledge sets, making the clear exchange of this distinct information indispensable. Structured formats, which provide an organized method of presenting information, are also prevalent. These formats enhance the comprehensibility and accessibility of the content. Contrasting this with the use of NL, we observe that the LLM-decided formats tend to be more direct and clear, effectively reducing redundancy.

\textbf{Brevity and Efficiency.}
Another prominent feature is the focus on brevity, underlining efficiency in communication. The formats chosen by LLMs often omit elements typically associated with human interaction, such as conventional pleasantries or emotive expressions, resulting in more concise exchanges. This brevity not only conserves computational resources but also concentrates the dialogue on the task at hand. By eliminating extraneous elements, the agents optimize the communication process, leading to faster and more efficient information exchange. This could be beneficial in scenarios where rapid and effective decision-making is paramount.

\subsection{RQ5: Alignment with Conventional Agent Communication Languages}
\label{sec:analysis-comm-acl}
RQ5 probes the extent to which the communication formats determined by LLMs using AutoForm align with traditional Agent Communication Languages (ACLs), such as KQML \citep{DBLP:conf/cikm/FininFMM94} and FIPA-ACL \citep{fipa_acl_messag_struc_specif}. These ACLs have been instrumental in structuring communication between intelligent agents to foster cooperation and coordination. A typical KQML message, as shown below, exemplifies the structured nature of traditional ACLs:

{\small\begin{verbatim}
(ask-one
  :sender joe
  :content (PRICE IBM ?price)
  :receiver stock-server
  :reply-with ibm-stock
  :language LPROLOG
  :ontology NYSE-TICKS)
\end{verbatim}
}

Our examination of the communication patterns emerging from AutoForm reveals an interesting resemblance to these structured elements. As depicted in~\cref{fig:case}, LLMs frequently employ a structured format where "@" denotes the \textit{receiver}, verb phrases such as "ContextCheck" indicate the \textit{performative} (the \textit{"ask-one"} in the above example), and a succinct text string encapsulates the \textit{content}. This structuring mirrors the composition of ACL messages, where each part serves a specific function in the communication process.

Intrigued by this similarity, we conduct an experiment where LLMs are prompted to communicate using a format similar to KQML:

{\small\begin{verbatim}
(performative
  :content ...
  :receiver ...)
\end{verbatim}
}
The results of this experiment on two GPT-4-based agents are presented in~\cref{tab:multi-rusults-conventional-acl}. We have two settings, one prompts the LLMs to use the exact KQML format as presented above, and the other setting uses the JSON version of KQML format, considering that LLMs may be more adept at JSON. While both settings show worse or comparable performance to AutoForm in terms of RougeL, the number of tokens consumed is larger than AutoForm. This finding suggests that while LLMs can indeed emulate the formality of traditional ACL formats, the AutoForm approach optimizes the communication by enhancing clarity and structure, yet concurrently reduces token usage.

\input{tables/multi-results-conventional-acl}
The implications of these results are twofold. Firstly, they affirm the potential of AutoForm in generating communication patterns that parallel the formal structures of established ACLs. Secondly, they demonstrate the efficiency of AutoForm in distilling the essence of these traditional formats into a more concise form, thereby conserving computational resources without sacrificing communicative effectiveness. This balance of clarity, structure, and brevity positions AutoForm as a powerful tool for facilitating intelligent agent communication in a variety of contexts.

==> tables/bk/multi-results-conventional-acl-bk.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{l*{6}{c}}
        \toprule
        & \multicolumn{3}{c}{\textbf{Hotpot QA}} & \multicolumn{3}{c}{\textbf{Multi Wiki}} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}
        \textbf{Model} &\textbf{Rougel} & \textbf{\#Tokens} & \textbf{$\Delta$ Tokens} &\textbf{Rougel} & \textbf{\#Tokens} & \textbf{$\Delta$ Tokens}\\
        \midrule
        kqml & 0.76 &313.76 &- &0.53 &368.08 & -\\
        \midrule
        json & 0.71 & 346.03 & +10.2\% &0.53 & 291.4 &-20.8\%\\
        \midrule
        AutoMed & 0.76 & 115.0 & -63.3\% &0.52 & 115.0 &-68.8\%\\
        \bottomrule
    \end{tabular}
    \caption{Multi-agent communication performances using conventional ACL format.}
    \label{tab:multi-rusults-conventional-acl}
    \vspace{-1.3em}
\end{table*}


==> tables/examples/hotpot_qa_example.tex <==
% \input{tables/examples/hotpot-qa-case/gpt-3.5}
% \input{tables/examples/hotpot-qa-case/gpt-3.5-4}
% \input{tables/examples/hotpot-qa-case/gpt-4-3.5}
% \input{tables/examples/hotpot-qa-case/gpt-4}

==> tables/examples/narrative_qa_example.tex <==
% \input{tables/examples/narrative-qa-case/gpt-3.5}
% \input{tables/examples/narrative-qa-case/gpt-3.5-4}
% \input{tables/examples/narrative-qa-case/gpt-4-3.5}
% \input{tables/examples/narrative-qa-case/gpt-4}


==> tables/examples/wiki_hop_example.tex <==
% \input{tables/examples/wiki-hop-case/gpt-3.5}
% \input{tables/examples/wiki-hop-case/gpt-3.5-4}
% \input{tables/examples/wiki-hop-case/gpt-4-3.5}
% \input{tables/examples/wiki-hop-case/gpt-4}


==> tables/prompt_table/aqua_tool_single_prompt.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{p{\linewidth}}
        \toprule
        \underline{\textbf{\textsc{Prompt for AQuA$_\text{tool}$}}} \\
        \vspace{-2mm}
        \textbf{CoT:} \\  
    Solve the problem presented below:\\
    ---\\
    \$\{task\_description\} \\
    ---\\\\
    
    RESPONSE GUIDELINES:\\
    1. Think step by step.\\
    2. Concluding with the Answer (Optional): End your response with "Answer: \{answer\}", where \{answer\} is the final result of your problem-solving process. The \{answer\} should be a single capital letter.\\
    3. You can use tools to execute Python code to help you do some calculations. You should not finish the whole problem in the code.\\
    4. Only when you end your response with "Answer: \{answer\}" will the dialogue end.\\
        \vspace{2mm}
        \textbf{AutoForm:}\\
        Solve the problem presented below:\\
---\\
\$\{task\_description\}\\
---\\\\

RESPONSE GUIDELINES:\\
1. Initial State Representation: Begin by providing a clear and detailed representation of the initial state or conditions of the problem. It could be code, pseudocode, JSON, markdown table, logical operators, or math equation.\\
2. Step-by-Step Solution Process: Progressively update the state representation as you work through each step of the solution. This should include all logical reasoning and calculations leading to the final answer.\\
3. Concluding with the Answer (Optional): End your response with "Answer: \{answer\}", where \{answer\} is the final result of your problem-solving process. The {answer} should be a single capital letter.\\
4. You can use tools to execute Python code to help you do some calculations. You should not finish the whole problem in the code.\\
5. Only when you end your response with "Answer: \{answer\}" will the dialogue end.\\
        \vspace{2mm}
        \textbf{Tool:}\\
        \vspace{-3mm}
\begin{verbatim}
{
  "name": "exec_python",
  "description": "Execute a Python script.",
  "parameters": {
    "type": "object",
    "properties": {
      "code": {
        "type": "string",
        "description": "The Python code to execute. The code should print the result to stdout.",
      },
    },
    "required": ["code"],
  },
}
\end{verbatim}
\vspace{-5mm}\\
        \bottomrule
    \end{tabular}
    \caption{
       Prompt for AQuA$_\text{tool}$
    }
    \label{tab:prompt-for-aqua-tool}
\end{table*}

==> tables/prompt_table/minute_qa_multi_prompt.tex <==
\begin{table*}
    \centering
    \small
    \caption{prompt for minute qa (multi)}
    \begin{tabular}{p{\linewidth}}
         \toprule
         \underline{\textbf{\textsc{prompt for minute qa (multi)}}}\\
         \textbf{4+ AutoMed:}\\
     You are \$\{agent\_name\}. Together with \$\{all\_roles\}, your objective is to collaboratively solve the problem presented below:\\
    ---\\
    \$\{task\_description\}\\
    ---\\

    RESPONSE GUIDELINES:\\
    1. Initial State Representation: Begin by providing a clear and detailed representation of the initial state or conditions of the problem. Explain it to make sure the other member understand it.\\
    2. Step-by-Step Solution Process: Progressively update the state representation as you work through each step of the solution. This should include all logical reasoning and calculations leading to the final answer.\\
    3. Your response should represent only a single turn of you in the conversation. It should also be short and contain as much information as possible.\\
    4. Check other member's answer by examining the reasoning process. Correct it if it's wrong.\\
    5. Make each turn informative to reduce the number of total turns.\\
    6. Since you and others are intelligent agents rather than human, you have your own communication form. At the beginning of the conversation, specify the communication form to optimize your interactions. It can be code, emoji, structured language, hybrid of different forms, etc. Prioritize efficiency and effectiveness in your communication form.\\
    7. Add your name as the prefix of your response.\\
    8. Please believe that the evidence in the question is sufficient, and the ultimate answer is definitely among the given options.\\
    REMEMBER:\\
    1.You should collaborate with your teammates to complete this task. For the work they have already completed, you don't need to redo it; you just need to continue from where they left off or point out any logical errors in their reasoning. \\
    2.IMPORTANT:Even though you are collaborating, you should maintain your rationality and boldly point out any errors in your teammates' reasoning. \\
    3.IMPORTANT:However, be careful not to mistake correct information as incorrect.\\
    4.IMPORTANT!!!:Since you and others are intelligent agents rather than human, you have your own communication form. At the beginning of the conversation, specify the communication form to optimize your interactions. It can be code, emoji, structured language, hybrid of different forms, etc. Prioritize efficiency and effectiveness in your communication form.\\
    5.If you think you have getted the final answer to the quesetion ,end your response with "Answer: \{answer\}", where \{answer\} is the final answer to the question and it can only be the choices in the end of the question.\\
    \vspace{2mm}
    \textbf{4+AutoMed+internal}
    RESPONSE GUIDELINES:\\
    1. Initial State Representation: Begin by providing a clear and detailed representation of the initial state or conditions of the problem. Explain it to make sure the other member understand it.\\
    2. Step-by-Step Solution Process: Progressively update the state representation as you work through each step of the solution. This should include all logical reasoning and calculations leading to the final answer.\\
    3. Your response should represent only a single turn of you in the conversation. It should also be short and contain as much information as possible.\\
    4. Check other member's answer by examining the reasoning process. Correct it if it's wrong.\\
    5. Make each turn informative to reduce the number of total turns.\\
    6. Add your name as the prefix of your response.\\
    7. Please believe that the evidence in the question is sufficient, and the ultimate answer is definitely among the given options.\\
    8. You should collaborate with your teammates to complete this task. For the work they have already completed, you don't need to redo it; you just need to continue from where they left off or point out any logical errors in their reasoning. \\
    9. Even though you are collaborating, you should maintain your rationality and boldly point out any errors in your teammates' reasoning. \\
    10.IMPORTANT:However, be careful not to mistake correct information as incorrect.\\
    11.IMPORTANT!!!:Since you and others are intelligent agents rather than human, you have your own communication form. At the beginning of the conversation, specify the communication form to optimize your interactions. It can be code, emoji, structured language, hybrid of different forms, etc. Prioritize efficiency and effectiveness in your communication form.\\
    12.If you think you have getted the final answer to the quesetion ,end your response with "Answer: {answer}", where {answer} is the final answer to the question and it can only be the choices in the end of the question.\\
    13.IMPORTANT:Do not repeatedly output the same thing in communication when disputes arise\\
    OUTPUT FORMAT:\\
    <begin>\\
    Thinking: {the task representation in your mind, this won't be shown to others}\\
    Speaking: {your response that follows the guidelines above(IMPORTANT!!!:Since you and others are intelligent agents rather than human, you have your own communication form. At the beginning of the conversation, specify the communication form to optimize your interactions. It can be code, emoji, structured language, hybrid of different forms, etc. Prioritize efficiency and effectiveness in your communication form.)}\\
    <end>\\
         \bottomrule
    \end{tabular}
    \label{tab:appendix-minute-qa-multi-prompt}
\end{table*}
